Positivity from J-Basis Operators in the Standard Model Effective Field Theory

In the effective field theory (EFT), the positivity bound on dim-8 effective operators tells us that the $s^2$ contribution in the scattering amplitude of 2-to-2 process geometrically corresponds to the convex cone composed of the ultraviolet (UV) states as the external rays. The J-Basis method can provide a complete group theory decomposition of the scattering amplitude on the direct product of the gauge group and the Lorentz group, thus to search for all UV states. Compared to previous methods, which can only perform direct product decomposition on the gauge groups, the J-Basis method greatly improves the strictness of the restrictions and also provides a systematic scheme for calculating the positivity bounds of the dim-8 operators.

==> aaa.tex <==
\appendix
\section{Matching Results}

In fact the J-basis idea only provide the possibility of UV particles' existing. We need to write out UV -SM interaction and calculate UV-EFT matching results to crosscheck. We list all calculation of 4Higgs ,4W and 4Fermions scattering process in Appendix.
\subsection{SM Higgs}
First we consider the initial state and final state as
$\left\{H_1, H_2\right\},\left\{H_3^{\dagger}, H_4^{\dagger}\right\}$, That is, the UV Lagrangian has the form $HHX$.

\textbf{UV states} $\left(\right.$$Spin$,$\left.SU(2)_w,U(1)_y\right)=(2,3,1): g M^{-1} \mathcal{H}_1^{\mu \nu I \dagger}\left(\partial_\mu H^T \epsilon \tau^I \partial_\nu H\right)+$ h.c.
$$
\begin{aligned}
& -e^{j m}\left(\tau^I\right)_m^i\left(\tau^I\right)_l^n \epsilon_{n k}\left(i \frac{g}{M}\right)^2\left(\frac{1}{i}\right)^4\left(p_{2 \mu} p_{1 \nu}\right)\left(p_{4 \lambda} p_{3 \sigma}\right) \frac{i\left(G_{\mu \lambda} G_{v \sigma}+G_{\mu \sigma} G_{v \lambda}-\frac{2}{3} G_{\mu \nu} G_{\lambda \sigma}\right)}{s_{13}-M^2} \\
& +\{i \leftrightarrow j, 1 \leftrightarrow 2\}+\{k \leftrightarrow l, 3 \leftrightarrow 4\}+\{i \leftrightarrow j, 1 \leftrightarrow 2, k \leftrightarrow l, 3 \leftrightarrow 4\} \\
& =\quad-i \frac{2 g^2}{4 M^4}\left(\epsilon^{j m}\left(\tau^I\right)_m^i\left(\tau^I\right)_l^n \epsilon_{n k}\left(s_{13}^2+s_{14}^2-\frac{2}{3} s_{12}^2\right)+\epsilon^{j m}\left(\tau^I\right)_m^i\left(\tau^I\right)_k^n \epsilon_{n l}\left(s_{14}^2+s_{13}^2-\frac{2}{3} s_{12}^2\right)\right)+\cdots \\
& =\quad i \frac{g^2}{M^4}\left(\delta_k^i \delta_l^j+\delta_l^i \delta_k^j\right)\left(s_{13}^2+s_{14}^2-\frac{2}{3} s_{12}^2\right)+\cdots \\
& =i \frac{8 g^2}{3 M^4}\left(\begin{array}{lll}
3 & -2 & 3
\end{array}\right)\left(\begin{array}{l}
\mathcal{M}_{D^4 H^2 H^{+2}}^{(1)} \\
\mathcal{M}_{D^4 H^2 H^2} \\
\mathcal{M}_{D^4 H^2 H^{+2}}^{(3)}
\end{array}\right)+\cdots \\
& =i \frac{8 g^2}{3 M^4}\left(\begin{array}{lll}
1 & 6 & 6
\end{array}\right)\left(\begin{array}{l}
\mathcal{M}_{D^4 H^2 H^{+2}, 1}^{(p)} \\
\mathcal{M}_{D^4 H^2 H^{+}, 2} \\
\mathcal{M}_{D^4 H^2 H^{+2}, 3}^{(p)}
\end{array}\right)+\cdots \,.\\
&
\end{aligned}
$$
\textbf{UV states} $\left(\right.$$Spin$,$\left.SU(2)_w,U(1)_y\right)=(1,3,1): g \mathcal{W}_1^{\mu I}\left(H^T \epsilon \tau^I i \stackrel{\leftrightarrow}{D}_\mu H\right)+$ h.c.
$$
\begin{aligned}
& -\epsilon^{j m}\left(\tau^I\right)_m^i\left(\tau^I\right)_k^n \epsilon_{n l}(i g)^2\left(p_1-p_2\right)_\mu\left(p_3-p_4\right)_\nu \frac{i}{-s_{12}-M^2}\left(-g^{\mu \nu}+\frac{\left(p_1+p_2\right)^\mu\left(p_1+p_2\right)^\nu}{M^2}\right)+\text { perms } \\
= & i \frac{2 g^2}{M^4}\left(e^{j m}\left(\tau^I\right)_m^i\left(\tau^I\right)_k^n \epsilon_{n l}\left(s_{13}^2-s_{14}^2\right)+\epsilon^{j m}\left(\tau^I\right)_m^i\left(\tau^I\right)_l^n \epsilon_{n k}\left(s_{14}^2-s_{13}^2\right)\right)+\cdots \\
= & 0
\end{aligned}
$$
\textbf{UV states}$\left(\right.$$Spin$,$\left.SU(2)_w,U(1)_y\right)=(0,3,1): g M \Xi_1^{I \dagger}\left(H^T \epsilon \tau^I H\right)+$ h.c.
$$
$$Considering that,$$
$$
\begin{aligned}
     \left(H_j \epsilon^{j k}\left(\tau^I\right)_k^i H_i\right)^{\dagger}=- & \left(H^{\dagger i}\left(\tau^I\right)_i^k \epsilon_{k j} H^{\dagger j}\right)
\end{aligned}
$$
$$
We have:$$
$$
$$
\begin{aligned}
& -\epsilon^{j m}\left(\tau^I\right)_m^i\left(\tau^I\right)_l^n \epsilon_{n k}(i g M)^2 \frac{i}{s_{12}-M^2}+\text { perms } \\
= & -i \frac{2 g^2}{M^4}\left(\epsilon^{j m}\left(\tau^I\right)_m^i\left(\tau^I\right)_l^n \epsilon_{n k}+\epsilon^{j m}\left(\tau^I\right)_m^i\left(\tau^I\right)_k^n \epsilon_{n l}\right) s_{12}^2+\cdots \\
= & i \frac{4 g^2}{M^4}\left(\delta_k^i \delta_l^j+\delta_l^i \delta_k^j\right) s_{12}^2+\cdots\\
& =\quad i \frac{32 g^2}{M^4}\left(\begin{array}{lll}
0 & 1 & 0
\end{array}\right)\left(\begin{array}{l}
\mathcal{M}_{D^4 H^2 H^{\dagger}}^{(1)} \\
\mathcal{M}_{D^4 H^2 H^{\dagger}} \\
\mathcal{M}_{D^4 H^2 H^{\dagger}}^{(3)}
\end{array}\right)+\cdots \\
& =\quad i \frac{32 g^2}{M^4}\left(\begin{array}{lll}
1 & 0 & 0
\end{array}\right)\left(\begin{array}{l}
\mathcal{M}_{D^4 H^2 H^{\dagger 2}, 1}^{(p)} \\
\mathcal{M}_{D^4 H^2 H^{\dagger} 2,2} \\
\mathcal{M}_{D^4 H^2 H^{\dagger} 2,3}
\end{array}\right)+\cdots \\
& \textbf{UV states}\left(Spin, S U(2)_w, U(1)_y\right)=(1,1,1): g \mathcal{B}_1^{\mu \dagger}\left(H^T \epsilon i \stackrel{\leftrightarrow}{D}_\mu H\right)+\text { h.c. } \\
& \left(H_j \epsilon^{j i} i \stackrel{\leftrightarrow}{D_\mu} H_i\right)^{\dagger}=i\left(D_\mu H^{\dagger i} \epsilon_{i j} H^{\dagger j}-H^{\dagger i} \epsilon_{i j} D_\mu H^{\dagger j}\right)=-H^{\dagger i} \epsilon_{i j} i \stackrel{\leftrightarrow}{D}_\mu H^{\dagger j} \\
& -\epsilon^{j i} \epsilon_{l k}(i g)^2\left(p_1-p_2\right)_\mu\left(p_3-p_4\right)_\nu \frac{i}{s_{12}-M^2}\left(-g^{\mu \nu}+\frac{\left(p_1+p_2\right)^\mu\left(p_1+p_2\right)^\nu}{M^2}\right)+\text { perms } \\
& =\quad-i \frac{2 g^2}{M^4}\left(\epsilon^{j i} \epsilon_{l k}\left(s_{13}^2-s_{14}^2\right)+\epsilon^{j i} \epsilon_{k l}\left(s_{14}^2-s_{13}^2\right)\right)+\cdots \\
& =\quad-i \frac{4 g^2}{M^4} \epsilon^{j i} \epsilon_{l k}\left(s_{13}^2-s_{14}^2\right)+\cdots \\
& =\quad i \frac{4 g^2}{M^4}\left(-\delta_k^i \delta_l^j+\delta_l^i \delta_k^j\right)\left(s_{13}^2-s_{14}^2\right)+\cdots \\
& =i \frac{32 g^2}{M^4}\left(\begin{array}{lll}
1 & 0 & -1
\end{array}\right)\left(\begin{array}{l}
\mathcal{M}_{D^4 H^2 H^{\dagger 2}}^{(1)} \\
\mathcal{M}_{D^4 H^2 H^{\dagger 2}} \\
\mathcal{M}_{D^4 H^2 H^{\dagger}}
\end{array}\right)+\cdots \\
& =\quad i \frac{32 g^2}{M^4}\left(\begin{array}{lll}
1 & 0 & 2
\end{array}\right)\left(\begin{array}{l}
\mathcal{M}_{D^4 H^2 H^{+2}, 1}^{(p)} \\
\mathcal{M}_{D^4 H^2 H^{\dagger}, 2}^{(p)} \\
\mathcal{M}_{D^4 H^2 H^{+2}, 3}^{(p)}
\end{array}\right)+\cdots \\
&
\end{aligned}
$$
\quad \quad Now we talked about coupling with the form $HH^{\dagger}X$, i.e $\left\{H_1, H_3^{\dagger}\right\},\left\{H_2, H_4^{\dagger}\right\}$
$$
$$
\textbf{UV states} ($Spin$,$\left.SU(2)_w,U(1)_y\right)=(2,3,0): g M^{-1} \mathcal{H}_0^{\mu \nu I}\left(\partial_\mu H^{\dagger} \tau^I \partial_\nu H\right)$
$$
\begin{aligned}
& \frac{1}{2}\left(\tau^I\right)_k^i\left(\tau^I\right)_l^j\left(i \frac{g}{M}\right)^2\left(\frac{1}{i}\right)^4\left(p_{3 \mu} p_{1 \nu}\right)\left(p_{4 \lambda} p_{2 \sigma}\right) \frac{i\left(G_{\mu \lambda} G_{v \sigma}+G_{\mu \sigma} G_{v \lambda}-\frac{2}{3} G_{\mu \nu} G_{\lambda \sigma}\right)}{s_{13}-M^2}+\text { perms } \\
& =\quad i \frac{g^2}{4 M^4}\left(\left(\tau^I\right)_k^i\left(\tau^I\right)_l^j\left(s_{12}^2+s_{14}^2-\frac{2}{3} s_{13}^2\right)+\left(\tau^I\right)_l^i\left(\tau^I\right)_k^j\left(s_{12}^2+s_{13}^2-\frac{2}{3} s_{14}^2\right)\right)+\cdots \\
& =\quad i \frac{g^2}{4 M^4}\left(\left(2 \delta_l^i \delta_k^j-\delta_k^i \delta_l^j\right)\left(s_{12}^2+s_{14}^2-\frac{2}{3} s_{13}^2\right)+\left(2 \delta_k^i \delta_l^j-\delta_l^i \delta_k^j\right)\left(s_{12}^2+s_{13}^2-\frac{2}{3} s_{14}^2\right)\right)+\cdots \\
& =\quad i \frac{g^2}{4 M^4}\left(\delta_k^i \delta_l^j\left(s_{12}^2-\frac{7}{3} s_{14}^2+\frac{8}{3} s_{13}^2\right)+\delta_l^i \delta_k^j\left(s_{12}^2-\frac{7}{3} s_{13}^2+\frac{8}{3} s_{14}^2\right)\right)+\cdots \\
& =\quad i \frac{2 g^2}{3 M^4}\left(\begin{array}{lll}
-7 & 3 & 8
\end{array}\right)\left(\begin{array}{l}
\mathcal{M}_{D^4 H^2 H^{\dagger 2}}^{(1)} \\
\mathcal{M}_{D^4 H^2 H^{\dagger}} \\
\mathcal{M}_{D^4 H^2 H^{\dagger}}^{(3}
\end{array}\right)+\cdots \\
& =\quad i \frac{2 g^2}{3 M^4}\left(\begin{array}{lll}
-4 & 1 & -14
\end{array}\right)\left(\begin{array}{l}
\mathcal{M}_{D^4 H^2 H^2, 1}^{(p)} \\
\mathcal{M}_{D^4 H^2 H^2, 2} \\
\mathcal{M}_{D^4 H^2 H^2, 3}
\end{array}\right)+\cdots \\
&
\end{aligned}
$$
\textbf{UV states}$\left(\right.$$Spin$,$\left.SU(2)_w,U(1)_y\right)=(1,3,0): g \mathcal{W}_0^{\mu I}\left(H^{\dagger} \tau^I i \stackrel{\leftrightarrow}{D_\mu} H\right)$
$$
\begin{aligned}
& \frac{1}{2}\left(\tau^I\right)_k^i\left(\tau^I\right)_l^j(i g)^2\left(p_3-p_1\right)_\mu\left(p_4-p_2\right)_\nu \frac{i}{s_{13}-M^2}\left(-g^{\mu \nu}+\frac{\left(p_1+p_3\right)^\mu\left(p_1+p_3\right)^\nu}{M^2}\right)+\text { perms } \\
& =\quad i \frac{g^2}{M^4}\left(\left(\tau^I\right)_k^i\left(\tau^I\right)_l^j\left(s_{12}^2-s_{14}^2\right)+\left(\tau^I\right)_l^i\left(\tau^I\right)_k^j\left(s_{12}^2-s_{13}^2\right)\right)+\cdots \\
& =i \frac{g^2}{M^4}\left(\left(2 \delta_l^i \delta_k^j-\delta_k^i \delta_l^j\right)\left(s_{12}^2-s_{14}^2\right)+\left(2 \delta_k^i \delta_l^j-\delta_l^i \delta_k^j\right)\left(s_{12}^2-s_{13}^2\right)\right)+\cdots \\
& =\quad i \frac{g^2}{M^4}\left(\delta_k^i \delta_l^j\left(s_{12}^2+s_{14}^2-2 s_{13}^2\right)+\delta_l^i \delta_k^j\left(s_{12}^2+s_{13}^2-2 s_{14}^2\right)\right)+\cdots \\
& =i \frac{8 g^2}{M^4}\left(\begin{array}{lll}
1 & 1 & -2
\end{array}\right)\left(\begin{array}{l}
\mathcal{M}_{D^4 H^2 H^{+2}}^{(1)} \\
\mathcal{M}_{D^4 H^2 H^{+2}} \\
\mathcal{M}_{D^4 H^2 H^{+2}}^{(3}
\end{array}\right)+\cdots \\
& =\quad i \frac{8 g^2}{M^4}\left(\begin{array}{lll}
2 & -1 & 2
\end{array}\right)\left(\begin{array}{l}
\mathcal{M}_{D^4 H^2 H^{+2}, 1}^{(p)} \\
\mathcal{M}_{D^4 H^2 H^{+2}, 2}^{(p)} \\
\mathcal{M}_{D^4 H^2 H^{+2}, 3}^{(p)}
\end{array}\right)+\cdots \\
&
\end{aligned}
$$
\textbf{UV states}$\left(Spin,SU(2)_w,U(1)_y\right)=(0,3,0): g M \Xi_0^I\left(H^{\dagger} \tau^I H\right)$
$$
\begin{aligned}
& \frac{1}{2}\left(\tau^I\right)_k^i\left(\tau^I\right)_l^j(i g M)^2 \frac{i}{-s_{13}-M^2}+\text { perms } \\
= & i \frac{g^2}{M^4}\left(\left(\tau^I\right)_k^i\left(\tau^I\right)_l^j s_{13}^2+\left(\tau^I\right)_l^i\left(\tau^I\right)_k^j s_{14}^2\right)+\cdots \\
= & i \frac{g^2}{M^4}\left(\left(2 \delta_l^i \delta_k^j-\delta_k^i \delta_l^j\right) s_{13}^2+\left(2 \delta_k^i \delta_l^j-\delta_l^i \delta_k^j\right) s_{14}^2\right)+\cdots \\
= & i \frac{g^2}{M^4}\left(\delta_k^i \delta_l^j\left(2 s_{14}^2-s_{13}^2\right)+\delta_l^i \delta_k^j\left(2 s_{13}^2-s_{14}^2\right)\right)+\cdots\\
& =i \frac{8 g^2}{M^4}\left(\begin{array}{lll}
2 & 0 & -1
\end{array}\right)\left(\begin{array}{l}
\mathcal{M}_{D^4 H^2 H^{\dagger}}^{(1)} \\
\mathcal{M}_{D^4 H^2 H^{\dagger}} \\
\mathcal{M}_{D^4 H^2 H^{\dagger}}^{(32}
\end{array}\right)+\cdots \\
& =i \frac{8 g^2}{M^4}\left(\begin{array}{lll}
2 & 1 & 4
\end{array}\right)\left(\begin{array}{l}
\mathcal{M}_{D^4 H^2 H^{+2}, 1}^{(p)} \\
\mathcal{M}_{D^4 H^2 H^{\dagger}, 2} \\
\mathcal{M}_{D^4 H^2 H^{+2}, 3}^{(p}
\end{array}\right)+\cdots \\
&
\end{aligned}
$$
\textbf{UV states}$\left(\right.$$Spin$,$\left.SU(2)_w,U(1)_y\right)=(2,1,0): g M^{-1} \mathcal{G}^{\mu \nu}\left(\partial_\mu H^{\dagger} \partial_\nu H\right)$
$$
\begin{aligned}
& \frac{1}{2} \delta_k^i \delta_l^j\left(i \frac{g}{M}\right)^2\left(\frac{1}{i}\right)^4\left(p_{3 \mu} p_{1 \nu}\right)\left(p_{4 \lambda} p_{2 \sigma}\right) \frac{i}{2} \frac{\left(G_{\mu \lambda} G_{v \sigma}+G_{\mu \sigma} G_{v \lambda}-\frac{2}{3} G_{\mu \nu} G_{\lambda \sigma}\right)}{s_{13}-M^2}+\text { perms } \\
& =\quad i \frac{g^2}{8 M^4}\left(\delta_k^i \delta_l^j\left(s_{12}^2+s_{14}^2-\frac{2}{3} s_{13}^2\right)+\delta_l^i \delta_k^j\left(s_{12}^2+s_{13}^2-\frac{2}{3} s_{14}^2\right)\right)+\cdots \\
& =\quad i \frac{g^2}{3 M^4}\left(\begin{array}{lll}
3 & 3 & -2
\end{array}\right)\left(\begin{array}{l}
\mathcal{M}_{D^4 H^2 H^{\dagger 2}}^{(1)} \\
\mathcal{M}_{D^4 H^2 H^{\dagger 2}} \\
\mathcal{M}_{D^4 H^2 H^{\dagger 2}}
\end{array}\right)+\cdots \\
& =\quad i \frac{g^2}{3 M^4}\left(\begin{array}{lll}
6 & 1 & 6
\end{array}\right)\left(\begin{array}{l}
\mathcal{M}_{D^4 H^2 H^{\dagger 2}, 1}^{(p)} \\
\mathcal{M}_{D^4 H^2 H^{\dagger}, 2}^{(2)} \\
\mathcal{M}_{D^4 H^2 H^{\dagger}, 3}^{(p)}
\end{array}\right)+\cdots 
\end{aligned}
$$
$$
$$\quad \quad However, we need to pay attention that in t channel, i.e $p_1\leftrightarrow p_3$, the amplitude doesn't have crossing symmetry, so we need to take another amplitude into consideration.$$
$$
$$
\begin{aligned}
& \frac{1}{2} \delta_k^i \delta_l^j\left(i \frac{g}{M}\right)^2\left(\frac{1}{i}\right)^4\left(p_{3 \mu} p_{1 \nu}\right)\left(p_{4 \lambda} p_{2 \sigma}\right) \frac{i}{2} \frac{\left(G_{\mu \lambda} G_{v \sigma}+G_{\mu \sigma} G_{v \lambda}-\frac{1}{2} G_{\mu \nu} G_{\lambda \sigma}\right)}{s_{13}-M^2}+\text { perms } \\
& =\quad i \frac{g^2}{8 M^4}\left(\delta_k^i \delta_l^j\left(s_{12}^2+s_{14}^2-\frac{1}{2} s_{13}^2\right)+\delta_l^i \delta_k^j\left(s_{12}^2+s_{13}^2-\frac{1}{2} s_{14}^2\right)\right)+\cdots \\
& =\quad i \frac{g^2}{2 M^4}\left(\begin{array}{lll}
2 & 2 & -1
\end{array}\right)\left(\begin{array}{l}
\mathcal{M}_{D^4 H^2 H^{\dagger 2}}^{(1)} \\
\mathcal{M}_{D^4 H^2 H^{\dagger 2}} \\
\mathcal{M}_{D^4 H^2 H^{\dagger}}^{3(3}
\end{array}\right)+\cdots \\
& =\quad i \frac{g^2}{3 M^4}\left(\begin{array}{lll}
4 & 1 & 4
\end{array}\right)\left(\begin{array}{c}
\mathcal{M}_{D^4 H^2 H^{\dagger}, 1}^{(p)} \\
\mathcal{M}_{D^4 H^2 H^{\dagger}, 2}^{(2} \\
\mathcal{M}_{D^4 H^2 H^{\dagger}, 3}^{(p)}
\end{array}\right)+\cdots \\
&
\end{aligned}
$$
$$
\begin{aligned}
& \textbf {UV states}\left(Spin,SU(2)_w,U(1)_y\right)=(1,1,0): g \mathcal{B}_0^\mu\left(H^{\dagger} i \stackrel{\leftrightarrow}{D}_\mu H\right) \\
& \frac{1}{2} \delta_k^i \delta_l^j(i g)^2\left(p_3-p_1\right)_\mu\left(p_4-p_2\right)_\nu \frac{i}{-s_{13}-M^2}\left(-g^{\mu \nu}+\frac{\left(p_1+p_3\right)^\mu\left(p_1+p_3\right)^\nu}{M^2}\right)+\text { perms } \\
& =\quad i \frac{g^2}{M^4}\left(\delta_k^i \delta_l^j\left(s_{12}^2-s_{14}^2\right)+\delta_l^i \delta_k^j\left(s_{12}^2-s_{13}^2\right)\right)+\cdots \\
& =i \frac{8 g^2}{M^4}\left(\begin{array}{lll}
-1 & 1 & 0
\end{array}\right)\left(\begin{array}{l}
\mathcal{M}_{D^4 H^2 H^{\dagger 2}}^{(1)} \\
\mathcal{M}_{D^4 H^2 H^{\dagger 2}} \\
\mathcal{M}_{D^4 H^2 H^{\dagger}}^{(3)}
\end{array}\right)+\cdots \\
& =\quad i \frac{8 g^2}{M^4}\left(\begin{array}{lll}
0 & -1 & -2
\end{array}\right)\left(\begin{array}{l}
\mathcal{M}_{D^4 H^2 H^{+2}, 1}^{(p)} \\
\mathcal{M}_{D^4 H^2 H^2, 2} \\
\mathcal{M}_{D^4 H^2 H^{\dagger}, 3}^{(p)}
\end{array}\right)+\cdots \\
&
\end{aligned}
$$
\textbf{UV states}$\left(Spin, S U(2)_w, U(1)_y\right)=(0,1,0): g M \mathcal{S}\left(H^{\dagger} H\right)$
$$
\begin{aligned}
& \frac{1}{2} \delta_k^i \delta_l^j(i g M)^2 \frac{i}{-s_{13}-M^2}+\text { perms } \\
& =i g^2\left[\delta_k^i \delta_l^j\left(1+\frac{s_{13}}{M^2}+\frac{s_{13}^2}{M^4}\right)+\delta_l^i \delta_k^j\left(1+\frac{s_{14}}{M^2}+\frac{s_{14}^2}{M^4}\right)\right]+\cdots \\
& =\quad i \frac{g^2}{M^4}\left(\delta_k^i \delta_l^j s_{13}^2+\delta_l^i \delta_k^j s_{14}^2\right)+\cdots \\
& =i \frac{8 g^2}{M^4}\left(\begin{array}{lll}
0 & 0 & 1
\end{array}\right)\left(\begin{array}{l}
\mathcal{M}_{D^4 H^2 H^{\dagger 2}}^{(1)} \\
\mathcal{M}_{D^4 H^2 H^{\dagger 2}}^{(2)} \\
\mathcal{M}_{D^4 H^2 H^{\dagger 2}}^{(3)}
\end{array}\right)+\cdots \\
& =i \frac{8 g^2}{M^4}\left(\begin{array}{lll}
0 & 1 & 0
\end{array}\right)\left(\begin{array}{l}
\mathcal{M}_{D^4 H^2 H^{\dagger 2}, 1}^{(p)} \\
\mathcal{M}_{D^4 H^2 H^{\dagger}, 2}^{(p)} \\
\mathcal{M}_{D^4 H^2 H^{\dagger}, 3}^{(p)}
\end{array}\right)+\cdots \\
&
\end{aligned}
$$
\subsection{$W$ vector}
\textbf{Scalar term:}\\
\textbf{UV states}$\left(Spin,SU(3)_c,SU(2)_w,U(1)_y\right)=(0,1,1,0): W_{\mathrm{L} \mu \nu}^I W_{\mathrm{L}}^{I \mu \nu} S+$ h.c.
$$
\mathcal{L}_{\mathrm{UV}}=-\frac{1}{2} S\left(\square+M^2\right) S+g W_{\mathrm{L} \mu \nu}^I W_{\mathrm{L}}^{I \mu \nu} S+g^* W_{\mathrm{R} \mu \nu}^I W_{\mathrm{R}}^{I \mu \nu} S\nonumber
$$
$W^2_{L}W^2_{R}$\\
The EOM of $S$ :
$$
\begin{aligned}
 S&=\frac{g W_{\mathrm{L} \mu \nu}^I W_{\mathrm{L}}^{I \mu \nu}+g^* W_{\mathrm{R} \mu \nu}^I W_{\mathrm{R}}^{I \mu \nu}}{\square+M^2} \\
\mathcal{L}_{\mathrm{EFT}}&=\frac{g g^*}{M^2} W_{\mathrm{L} \mu \nu}^I W_{\mathrm{L}}^{I \mu \nu} W_{\mathrm{R} \rho \lambda}^J W_{\mathrm{R}}^{J \rho \lambda} \\
& =\frac{4 g g^*}{M^2}\left(\begin{array}{ll}
0 & -1
\end{array}\right)\left(\begin{array}{l}
\mathcal{O}_{W_{\mathrm{L}}^2 W_{\mathrm{R}}^2, 1}^{(p)} \\
\mathcal{O}_{W_{\mathrm{L}}^2 W_{\mathrm{R}}^2, 2}^2
\end{array}\right) \\
&
\end{aligned}
$$
$W^4_{L}$\\
The EOM of $S$ :
$$
\begin{aligned}
 S&=\frac{g W_{\mathrm{L} \mu \nu}^I W_{\mathrm{L}}^{I \mu \nu}}{\square+M^2} \\
 \mathcal{L}_{\mathrm{EFT}}&= \frac{g^2}{2 M^2} W_{\mathrm{L} \mu \nu}^I W_{\mathrm{L}}^{I \mu \nu} W_{\mathrm{L} \rho \lambda}^J W_{\mathrm{L}}^{J \rho \lambda} \\
&= \frac{2 g^2}{M^2}\left(\begin{array}{ll}
-1 & 0
\end{array}\right)\left(\begin{array}{l}
\mathcal{O}_{W_{\mathrm{L}}^{(p)}, 1}^{(p)} \\
\mathcal{O}_{W_{\mathrm{L}}^4, 2}^{(p)}
\end{array}\right)
\end{aligned}
$$
\\
\\
\textbf{UV states}$\left(\right.$$Spin$,$\left.SU(3)_c, SU(2)_w,U(1)_y\right)=(0, \mathbf{1}, \mathbf{5}, 0): W_{\mathrm{L} \mu \nu}^I W_{\mathrm{L}}^{J \mu \nu}\left(T^{\Lambda}\right)^{I J} \mathcal{S}^{\Lambda}+$ h.c.
$$
\mathcal{L}_{\mathrm{UV}}=-\frac{1}{2} S^{\Lambda}\left(\square+M^2\right) S^{\Lambda}+g W_{\mathrm{L} \mu \nu}^I W_{\mathrm{L}}^{J \mu \nu}\left(T^{\Lambda}\right)^{I J} \mathcal{S}^{\Lambda}+g^* W_{\mathrm{R} \mu \nu}^I W_{\mathrm{R}}^{J \mu \nu}\left(T^{\Lambda}\right)^{I J} \mathcal{S}^{\Lambda}
$$
$W^2_{L}W^2_{R}$\\
The EOM of $S^{\Lambda}$ :
$$
\begin{aligned}
 S^{\Lambda}&=\frac{g W_{\mathrm{L} \mu \nu}^I W_{\mathrm{L}}^{J \mu \nu}\left(T^{\Lambda}\right)^{I J}+g^* W_{\mathrm{R}}^I{ }^{\mu \nu} W_{\mathrm{R}}^{J \mu \nu}\left(T^{\Lambda}\right)^{I J}}{\square+M^2} \\
\mathcal{L}_{\mathrm{EFT}} & =\frac{g g^*}{M^2} W_{\mathrm{L} \mu \nu}^I W_{\mathrm{L}}^{J \mu \nu} W_{\mathrm{R} \rho \lambda}^K W_{\mathrm{R}}^{L \rho \lambda}\left(T^{\Lambda}\right)^{I J}\left(T^{\Lambda}\right)^{K L} \\
& =\frac{g g^*}{2 M^2} W_{\mathrm{L} \mu \nu}^I W_{\mathrm{L}}^{J \mu \nu} W_{\mathrm{R} \rho \lambda}^K W_{\mathrm{R}}^{L \rho \lambda}\left(\delta^{I K} \delta^{J L}+\delta^{I L} \delta^{J K}-\frac{2}{3} \delta^{I J} \delta^{K L}\right) \\
& =\frac{4 g g^*}{3 M^2}\left(\begin{array}{ll}
-3 & 1
\end{array}\right)\left(\begin{array}{c}
\mathcal{O}_{W_{\mathrm{L}}^2 W_{\mathrm{R}}^2, 1}^{(p)} \\
\mathcal{O}_{W_{\mathrm{L}}^2 W_{\mathrm{R}}^2, 2}
\end{array}\right)
\end{aligned}
$$
$W^4_{L}$\\
The EOM of $S^{\Lambda}$ :
$$
\begin{aligned}
 S^{\Lambda}&=\frac{g W_{\mathrm{L} \mu \nu}^I W_{\mathrm{L}}^{J \mu \nu}\left(T^{\Lambda}\right)^{I J}}{\square+M^2} \\
 \mathcal{L}_{\mathrm{EFT}}&=\frac{g^2}{2 M^2} W_{\mathrm{L} \mu \nu}^I W_{\mathrm{L}}^{J \mu \nu} W_{\mathrm{L} \rho \lambda}^K W_{\mathrm{L}}^{L \rho \lambda}\left(T^{\Lambda}\right)^{I J}\left(T^{\Lambda}\right)^{K L} \\
&=\frac{g^2}{2 M^2} W_{\mathrm{L} \mu \nu}^I W_{\mathrm{L}}^{J \mu \nu} W_{\mathrm{L} \rho \lambda}^K W_{\mathrm{L}}^{L \rho \lambda}\left(\delta^{I K} \delta^{J L}+\delta^{I L} \delta^{J K}-\frac{2}{3} \delta^{I J} \delta^{K L}\right) \\
&=\frac{g^2}{3 M^2}\left(\begin{array}{ll}
4 & 3
\end{array}\right)\left(\begin{array}{c}
\mathcal{O}_{W_{\mathrm{L}}^4, 1}^{(p)} \\
\mathcal{O}_{W_{\mathrm{L}}^4, 2}^{(p)}
\end{array}\right)
\end{aligned}
$$\\
\quad \quad Massive spin-2 coupling:\\
\quad \quad We have already discussed, there exist only $W_{L}^2W_{R}^2$ terms.

\textbf{UV states}$\left(Spin,SU(3)_c,SU(2)_w,U(1)_y\right)=(2, \mathbf{1}, \mathbf{5}, 0): W_{\mathrm{L} \mu \nu}^I W_{\mathrm{R} \rho}^J{ }^\nu\left(T^{\Lambda}\right)^{I J} \mathcal{H}_5^{\Lambda \mu \rho}$
$$
\begin{aligned}
\mathcal{L}_{\mathrm{EFT}}= & \frac{g^2}{2 M^2}\left(g^{\mu \lambda} g^{\nu \rho}+g^{\nu \lambda} g^{\mu \rho}-\frac{2}{3} g^{\mu \nu} g^{\lambda \rho}\right)\left(\left(T^{\Lambda}\right)^{I J}\left(T^{\Lambda}\right)^{K L} W_{\mathrm{L} \mu \xi}^I W_{\mathrm{R} \nu}^J{ }^{\xi} W_{\mathrm{L} \lambda \sigma}^K W_{\mathrm{R} \rho}^L\right) \\
= & \frac{g^2}{2 M^2}\left(\delta^{I K} \delta^{J L}+\delta^{I L} \delta^{J K}-\frac{2}{3} \delta^{I J} \delta^{K L}\right)\left(W_{\mathrm{L} \mu \xi}^I W_{\mathrm{R}}^J{ }^{\xi} W_{\mathrm{L}}^{K \mu}{ }_\sigma W_{\mathrm{R}}^{L \nu \sigma}+W_{\mathrm{L} \mu \xi}^I W_{\mathrm{R} \nu}^J{ }^{\xi} W_{\mathrm{L}}^{K \nu}{ }_\sigma W_{\mathrm{R}}^{L \mu \sigma}\right. \\
& \left.-\frac{2}{3} W_{\mathrm{L} \mu \xi}^I W_{\mathrm{R}}^{J \mu \xi} W_{\mathrm{L} \lambda \sigma}^K W_{\mathrm{R}}^{L \lambda \sigma}\right) \\
= & \frac{g^2}{3 M^2}(-1-3)\left(\begin{array}{c}
\mathcal{O}_{W_{\mathrm{L}}^2}^{(p)} W_{\mathrm{R}}^2, 1 \\
\mathcal{O}_{\mathrm{L}}^{(p)} \\
W_{\mathrm{L}}^2 W_{\mathrm{R}}^2, 2
\end{array}\right)
\end{aligned}
$$
\textbf{UV states}$\left(Spin,SU(3)_c,SU(2)_w,U(1)_y\right)=(2,1,3,0): \epsilon_{I J K} W_{\mathrm{L} \mu \nu}^I W_{\mathrm{R} \rho}^J{ }^\nu \mathcal{H}_3^{K \mu \rho}$
$$
\begin{aligned}
 \mathcal{L}_{\mathrm{EFT}}&=\frac{g^2}{2 M^2}\left(g^{\mu \lambda} g^{\nu \rho}+g^{\nu \lambda} g^{\mu \rho}-\frac{2}{3} g^{\mu \nu} g^{\lambda \rho}\right)\left(\epsilon^{I J M} \epsilon^{K L M} W_{\mathrm{L} \mu \xi}^I W_{\mathrm{R} \nu}^J{ }^{\xi} W_{\mathrm{L}}^K \lambda \sigma W_{\mathrm{R} \rho}^L\right) \\
& =\frac{g^2}{2 M^2} \epsilon^{I J M} \epsilon^{K L M}\left(W_{\mathrm{L} \mu \xi}^I W_{\mathrm{R}}^J \nu^{\xi} W_{\mathrm{L}}^{K \mu}{ }_\sigma W_{\mathrm{R}}^{L \nu \sigma}+W_{\mathrm{L} \mu \xi}^I W_{\mathrm{R} \nu}^J{ }^{\xi} W_{\mathrm{L}}^{K \nu}{ }_\sigma W_{\mathrm{R}}^{L \mu \sigma}-\frac{2}{3} W_{\mathrm{L} \mu \xi}^I W_{\mathrm{R}}^{J \mu \xi} W_{\mathrm{L} \lambda \sigma}^K W_{\mathrm{R}}^{L \lambda \sigma}\right) \\
& =\frac{g^2}{M^2}\left(\begin{array}{ll}
1 & -1
\end{array}\right)\left(\begin{array}{c}
\mathcal{O}_{W_{\mathrm{L}}^2 W_{\mathrm{R}}^2, 1}^{(p)} \\
\mathcal{O}_{W_{\mathrm{L}}^2 W_{\mathrm{R}}^2, 2}^{(p)}
\end{array}\right) \\
&
\end{aligned}
$$
\textbf{UV states} $\left(Spin, S U(3)_c, S U(2)_w, U(1)_y\right)=(2, \mathbf{1}, \mathbf{1}, 0): W_{\mathrm{L} \mu \nu}^I W_{\mathrm{R} \rho}^I \mathcal{G}^{\mu \rho}$
$$
\mathcal{L}_{\mathrm{UV}}=-\frac{1}{2}\left(g^{\mu \lambda} g^{\nu \rho}+g^{\nu \lambda} g^{\mu \rho}-\frac{2}{3} g^{\mu \nu} g^{\lambda \rho}\right)^{-1} \mathcal{G}^{\mu \nu}\left(\square+M^2\right) \mathcal{G}^{\lambda \rho}+g W_{\mathrm{L} \lambda \sigma}^I W_{\mathrm{R} \rho}^I \mathcal{G}^{\lambda \rho}
$$
The EOM of $\mathcal{G}^{\mu \nu}:$
$$
\begin{aligned}
\mathcal{L}_{\mathrm{EFT}} & =\frac{g^2}{2 M^2}\left(g^{\mu \lambda} g^{\nu \rho}+g^{\nu \lambda} g^{\mu \rho}-\frac{2}{3} g^{\mu \nu} g^{\lambda \rho}\right)\left(W_{\mathrm{L} \mu \xi}^I W_{\mathrm{R} \nu}^I{ }^{\xi} W_{\mathrm{L} \lambda \sigma}^J W_{\mathrm{R} \rho}^J{ }^\sigma\right) \\
& =\frac{g^2}{2 M^2}\left(W_{\mathrm{L} \mu \xi}^I W_{\mathrm{R} \nu}^I{ }^{\xi} W_{\mathrm{L}}^{J \mu}{ }_\sigma W_{\mathrm{R}}^{J \nu \sigma}+W_{\mathrm{L} \mu \xi}^I W_{\mathrm{R} \nu}^I{ }^{\xi} W_{\mathrm{L}}^{J \nu}{ }_\sigma W_{\mathrm{R}}^{J \mu \sigma}-\frac{2}{3} W_{\mathrm{L} \mu \xi}^I W_{\mathrm{R}}^{I \mu \xi} W_{\mathrm{L} \lambda \sigma}^J W_{\mathrm{R}}^{J \lambda \sigma}\right) \\
& =\frac{g^2}{M^2}\left(\begin{array}{ll}
-1 & 0
\end{array}\right)\left(\begin{array}{c}
\mathcal{O}_{W_{\mathrm{L}}^2 W_{\mathrm{R}}^2, 1}^{(p)} \\
\mathcal{O}_{W_{\mathrm{L}}^2 W_{\mathrm{R}}^2, 2}^{(p)}
\end{array}\right)
\end{aligned}
$$
\subsection{Fermions with Generations}
\textbf{UV states} $\left(Spin, S U(3)_c, S U(2)_w, U(1)_y\right)=(1,1,3,1): g_{p_1 p_2} \epsilon^{i_1 m}\left(\tau^I\right)_m^{i_2} \mathcal{W}_1^{\mu I}\left(L_{p_1 i_1} i \stackrel{\leftrightarrow}{D}_\mu L_{p_2 i_2}\right)+$ h.c.
$$
\mathcal{L}_{\mathrm{UV}}=\mathcal{W}_{1 \mu}^{\dagger I}\left(\square+M^2\right) \mathcal{W}_1^{\mu I}+g_{p_1 p_2} \epsilon^{i_1 m}\left(\tau^I\right)_m^{i_2} \mathcal{W}_1^{\mu I}\left(L_{p_1 i_1} i \stackrel{\leftrightarrow}{D}_\mu L_{p_2 i_2}\right)-g_{p_1 p_2}^*\left(\tau^I\right)_{i_2}^m \epsilon_{m i_1} \mathcal{W}_1^{\dagger \mu}\left(L_{p_2}^{\dagger i_2} i \stackrel{\leftrightarrow}{D_\mu} L_{p_1}^{\dagger i_1}\right)
$$
The EOM of $\mathcal{W}^{\mu I}$ :
$$
\begin{aligned}
& \left(\square+M^2\right) \mathcal{W}_{1 \mu}^I-g_{p_1 p_2}^*\left(\tau^I\right)_{i_2}^m \epsilon_{m i_1}\left(L_{p_2}^{\dagger_2} i \stackrel{\leftrightarrow}{D_\mu} L_{p_1}^{\dagger i_1}\right)=0, \\
& \mathcal{W}_{1 \mu}^I=\frac{g_{p_1 p_2}^*\left(\tau^I\right)_{i_2}^m \epsilon_{m i_1}\left(L_{p_2}^{\dagger i_2} i \stackrel{\leftrightarrow}{D}_\mu L_{p_1}^{\dagger i_1}\right)}{\left(\square+M^2\right)} . \\
&
\end{aligned}
$$
The EOM of $\mathcal{W}_1^{\dagger \mu I}$ :
$$
\begin{aligned}
 \mathcal{W}_{1 \mu}^{\dagger I}&=-\frac{g_{p_1 p_2} \epsilon^{i_1 m}\left(\tau^I\right)_m^{i_2}\left(L_{p_1 i_1} i \stackrel{\leftrightarrow}{D}_\mu L_{p_2 i_2}\right)}{\left(\square+M^2\right)} \\
 \mathcal{L}_{\mathrm{EFT}}&=\frac{g_{p_1 p_2} g_{p_3 p_4}^*}{M^2} \epsilon^{i_1 m}\left(\tau^I\right)_m^{i_2}\left(\tau^I\right)_{i_4}^n \epsilon_{n i_3}\left(L_{p_1 i_1} i \stackrel{\leftrightarrow}{D}_\mu L_{p_2 i_2}\right)\left(L_{p_4}^{\dagger_4} i \stackrel{\leftrightarrow}{D}{ }^\mu L_{p_3}^{\dagger i_3}\right) \\
& =-\frac{g_{p_1 p_2} g_{p_3 p_4}^*}{M^2} \epsilon^{i_1 m}\left(\tau^I\right)_m^{i_2}\left(\tau^I\right)_{i_4}^n \epsilon_{n i_3}\left(L_{p_1 i_1} i \stackrel{\leftrightarrow}{D}_\mu L_{p_2 i_2}\right)\left(L_{p_3}^{\dagger i_3} i \stackrel{\leftrightarrow}{D}{ }^\mu L_{p_4}^{\dagger i_4}\right) \\
& =-\frac{g_{p_1 p_2} g_{p_3 p_4}^*}{M^2} \epsilon^{i_{1 m}}\left(\tau^I\right)_m^{i_2}\left(\tau^I\right)_{{ }_4}^n \epsilon_{n i_3}(\langle 12\rangle\langle 14\rangle[14][34]-\langle 12\rangle\langle 13\rangle[13][34]) \\
& =\frac{g_{p_1 p_2} g_{p_3 p_4}^*}{M^2}\left(\delta_{i_3}^{i_1} \delta_{i_4}^{i_2}+\delta_{i_4}^{i_1} \delta_{i_3}^{i_2}\right)\left(-\langle 12\rangle\langle 34\rangle[34]^2+2\langle 13\rangle\langle 24\rangle[34]^2\right) \\
&
 =\frac{g_{p_1 p_2} g_{p_3 p_4}^*}{M^2}\left(\begin{array}{llll}
-1 & 2 & -1 & 2
\end{array}\right)\left(\begin{array}{l}
\mathcal{O}_{L^2 L^{\dagger 2} D^2, 1}^{(y)} \\
\mathcal{O}_{L^2 L^{\dagger 2} D^2, 2} \\
\mathcal{O}_{L^2 L^{\dagger 2} D^2, 3} \\
\mathcal{O}_{L^2 L^{\dagger 2} D^2, 4}^{(y)}
\end{array}\right) \\
& =\frac{g_{p_1 p_2} g_{p_3 p_4}^*}{M^2}\left(\begin{array}{llll}
0 & 0 & 0 & -4
\end{array}\right)\left(\begin{array}{l}
\mathcal{O}_{L^2 L^{\dagger 2} D^2, 1}^{(p)} \\
\mathcal{O}_{L^2 L^{\dagger 2} D^2, 2}^{(p)} \\
\mathcal{O}_{L^2 L^{\dagger 2} D^2, 3}^{(p)} \\
\mathcal{O}_{L^2 L^{\dagger 2} D^2, 4}^{(p}
\end{array}\right) \\
&
\end{aligned}
$$
\textbf{UV states}$\left(Spin, S U(3)_c, S U(2)_w, U(1)_y\right)=(0,1,3,1): g_{p_1 p_2} \epsilon^{i_1 m}\left(\tau^I\right)_m^{i_2} \Xi^I\left(L_{p_1 i_1} L_{p_2 i_2}\right)+$ h.c.
$$
\mathcal{L}_{\mathrm{UV}}=-\Xi^{\dagger I}\left(\square+M^2\right) \Xi^I+g_{p_1 p_2} \epsilon^{i_{1 m}}\left(\tau^I\right)_m^{i_2} \Xi^I\left(L_{p_1 i_1} L_{p_2 i_2}\right)-g_{p_1 p_2}^*\left(\tau^I\right)_{i_2}^m \epsilon_{m i_1} \Xi^{\dagger I}\left(L_{p_2}^{\dagger i_2} L_{p_1}^{\dagger i_1}\right)
$$
The EOM of $\Xi^I$ :
$$
\begin{gathered}
-\left(\square+M^2\right) \Xi^I-g_{p_1 p_2}^*\left(\tau^I\right)_{i_2}^m \epsilon_{m i_1}\left(L_{p_2}^{\dagger i_2} L_{p_1}^{\dagger i_1}\right)=0, \\
\Xi^I=-\frac{g_{p_1 p_2}^*\left(\tau^I\right)_{i_2}^m \epsilon_{m i_1}\left(L_{p_2}^{\dagger i_2} L_{p_1}^{\dagger i_1}\right)}{\left(\square+M^2\right)} .
\end{gathered}
$$
The EOM of $\Xi^{\dagger I}$ :
$$
\Xi^{\dagger I}=\frac{g_{p_1 p_2} \epsilon^{i_1 m}\left(\tau^I\right)_m^{i_2}\left(L_{p_1 i_1} L_{p_2 i_2}\right)}{\left(\square+M^2\right)} .
$$
After integrating out $\Xi^I$,
$$
\begin{aligned}
& =-\frac{g_{p_1 p_2} g_{p_3 p_4}^*}{M^4}\left(\begin{array}{llll}
4 & 0 & 0 & 0
\end{array}\right)\left(\begin{array}{l}
\mathcal{O}_{L^2 L^{\dagger 2} D^2, 1}^{(p)} \\
\mathcal{O}_{L^2 L^{\dagger 2} D^2, 2}^{(p)} \\
\mathcal{O}_{L^2 L^{\dagger 2} D^2, 3}^{(p)} \\
\mathcal{O}_{L^2 L^{\dagger 2} D^2, 4}^{(p)}
\end{array}\right) \\
&
\end{aligned}
$$
\textbf{UV states} $\left(\right.$ $Spin$, $\left.S U(3)_c, S U(2)_w, U(1)_y\right)=(1,1,1,1): g_{p_1 p_2} \epsilon^{i_1 i_2} \mathcal{B}_1^\mu\left(L_{p_1 i_1} i \stackrel{\leftrightarrow}{D}_\mu L_{p_2 i_2}\right)+$ h.c.
$$
\begin{aligned}
 \mathcal{L}_{\mathrm{EFT}}&=\frac{g_{p_1 p_2} g_{p_3 p_4}^*}{M^2} \epsilon^{i_1 i_2} \epsilon_{i_4 i_3}\left(L_{p_1 i_1} i \stackrel{\leftrightarrow}{D}_\mu L_{p_2 i_2}\right)\left(L_{p_4}^{i_4} i \stackrel{\leftrightarrow}{D}{ }^\mu L_{p_3}^{\dagger i_3}\right) \\
& =-\frac{g_{p_1 p_2} g_{p_3 p_4}^*}{M^2} \epsilon^{i_1 i_2} \epsilon_{i_4 i_3}\left(L_{p_1 i_1} i \stackrel{\leftrightarrow}{D_\mu} L_{p_2 i_2}\right)\left(L_{p_3}^{\dagger_3} i \stackrel{\leftrightarrow}{D}{ }^\mu L_{p_4}^{\dagger_4}\right) \\
& =-\frac{g_{p_1 p_2} g_{p_3 p_4}^*}{M^2} \epsilon^{i_1 i_2} \epsilon_{i_4 i_3}(\langle 12\rangle\langle 14\rangle[14][34]-\langle 12\rangle\langle 13\rangle[13][34]) \\
&
\end{aligned}
$$
\textbf{UV states} $\left(\right.$ $Spin$, $\left.S U(3)_c, S U(2)_w, U(1)_y\right)=(0,1,1,1): g_{p_1 p_2} \epsilon^{i_1 i_2} S\left(L_{p_1 i_1} L_{p_2 i_2}\right)+$ h.c.
$$
\begin{aligned}
 \mathcal{L}_{\mathrm{EFT}}&=\frac{g_{p_1 p_2} g_{p_3 p_4}^*}{M^4} \epsilon^{i_1 i_2} \epsilon_{i_4 i_3} \square\left(L_{p_1 i_1} L_{p_2 i_2}\right)\left(L_{p_4}^{\dagger i_4} L_{p_3}^{\dagger i_3}\right) \\
& =\frac{g_{p_1 p_2} g_{p_3 p_4}^*}{M^4} \epsilon^{i_1 i_2} \epsilon_{i_4 i_3}(\langle 12\rangle\langle 12\rangle[12][34]) \\
& =-\frac{g_{p_1 p_2} g_{p_3 p_4}^*}{M^4}\left(\delta_{i_3}^{i_1} \delta_{i_4}^{i_2}-\delta_{i_4}^{i_1} \delta_{i_3}^{i_2}\right)\langle 12\rangle\langle 34\rangle[34]^2 \\
& =\frac{g_{p_1 p_2} g_{p_3 p_4}^*}{M^4}\left(\begin{array}{llll}
-1 & 0 & 1 & 0
\end{array}\right)\left(\begin{array}{l}
\mathcal{O}_{L^2 L^{\dagger 2} D^2, 1}^{(y)} \\
\mathcal{O}_{L^2 L^{\dagger 2} D^2, 2}^{(2)} \\
\mathcal{O}_{L^2 L^{\dagger 2} D^2, 3} \\
\mathcal{O}_{L^2 L^{\dagger} D^2, 4}^{(y)}
\end{array}\right) \\
& =\frac{g_{p_1 p_2} g_{p_3 p_4}^*}{M^4}\left(\begin{array}{llll}
0 & 0 & -4 & 0
\end{array}\right)\left(\begin{array}{l}
\mathcal{O}_{L^2 L^{+2} D^2, 1}^{(p)} \\
\mathcal{O}_{L^2 L^{+2} D^2, 2}^{(p)} \\
\mathcal{O}_{L^2 \perp^{+2} D^2, 3}^{(p)} \\
\mathcal{O}_{L^2 L^{+2} D^2, 4}^{(p)}
\end{array}\right) \\
&
\end{aligned}
$$
\textbf{UV states} $\left(Spin, S U(3)_c, S U(2)_w, U(1)_y\right)=(2,1,3,0): g_{p 1 p_3}\left(\tau^I\right)_{i_3}^{i_1} \mathcal{H}^{\mu \nu I}\left(L_{p 1 i_1} i \sigma_\mu \stackrel{\leftrightarrow}{D}_\nu L_{p_3}^{i_3}\right)$
$$
\mathcal{L}_{\mathrm{UV}}=-\frac{1}{2}\left(g^{\mu \lambda} g^{\nu \rho}+g^{\nu \lambda} g^{\mu \rho}-\frac{2}{3} g^{\mu \nu} g^{\lambda \rho}\right)^{-1} \mathcal{H}^{\mu \nu I}\left(\square+M^2\right) \mathcal{H}^{\lambda \rho I}+g_{p_1 p_3}\left(\tau^I\right)_{i_3}^{i_1} \mathcal{H}^{\mu \nu I}\left(L_{p_1 i_1} i \sigma_\mu \stackrel{\leftrightarrow}{D}_\nu L_{p_3}^{\dagger i_3}\right)
$$
The EOM of $\mathcal{H}^{\mu \nu I}$ :
$$
\begin{aligned}
 \mathcal{H}^{\mu \nu I}&=\frac{\left(\tau^I\right)_{i_3}^{i_1}\left(g^{\mu \lambda} g^{\nu \rho}+g^{\nu \lambda} g^{\mu \rho}-\frac{2}{3} g^{\mu \nu} g^{\lambda \rho}\right)\left(L_{p_1 i_1} \sigma_\lambda \stackrel{\leftrightarrow}{D}_\rho L_{p_3}^{\dagger i_3}\right)}{\square+M^2} \\
 \mathcal{L}_{\mathrm{EFT}}&=\frac{g_{p_1 p_3} g_{p_2 p_4}}{2 M^2}\left(\tau^I\right)_{i_3}^{i_1}\left(\tau^I\right)_{i_4}^{i_2}\left(g^{\mu \lambda} g^{\nu \rho}+g^{\nu \lambda} g^{\mu \rho}-\frac{2}{3} g^{\mu \nu} g^{\lambda \rho}\right)\left(L_{p_1 i_1} i \sigma_\mu \stackrel{\leftrightarrow}{D}_\nu L_{p_3}^{i_3}\right)\left(L_{p_2 i_2} i \sigma_\lambda \stackrel{\leftrightarrow}{D}_\rho L_{p_4}^{\dagger i_4}\right) \\
& =\frac{g_{p_1 p_3} g_{p_2 p_4}}{2 M^2}\left(\tau^I\right)_{i_3}^{i_1}\left(\tau^I\right)_{i_4}^{i_2}\big[\left(L_{p_1 i_1} i \sigma_\mu \stackrel{\leftrightarrow}{D}_\nu L_{p_3}^{\dagger i_3}\right)\left(L_{p_{22} i_2} i \sigma^\mu \stackrel{\leftrightarrow}{D} L_{p_4}^{\dagger i_4}\right)+\\&
\left(L_{p_1 i_1} i \sigma_\mu \stackrel{\leftrightarrow}{D}_\nu L_{p_3}^{\dagger i_3}\right)\left(L_{p_2 i_2} i \sigma^\nu \stackrel{\leftrightarrow}{D} L_{p_4}^{\dagger i_4}\right)\big] \\
& =\frac{g_{p_1 p_3} g_{p_2 p_4}}{2 M^2}\left(\tau^I\right)_{i_3}^{i_1}\left(\tau^I\right)_{i_4}^{i_2}[2\langle 12\rangle[34](-\langle 12\rangle[12]+\langle 14\rangle[14]) \\
& -(\langle 14\rangle[43]\langle 23\rangle[34]-\langle 14\rangle[43]\langle 21\rangle[14]-\langle 12\rangle[23]\langle 23\rangle[34]+\langle 12\rangle[23]\langle 21\rangle[14])] \\
& =\frac{g_{p_1 p_3} g_{p_2 p_4}}{2 M^2}\left(2 \delta_{i_4}^{i_1} \delta_{i_3}^{i_2}-\delta_{i_3}^{i_1} \delta_{i_4}^{i_2}\right)\left(-8\langle 12\rangle\langle 34\rangle[34]^2+6\langle 13\rangle\langle 24\rangle[34]^2\right) \\
& =\frac{g_{p_1 p_3} g_{p_2 p_4}}{M^2}\left(\begin{array}{llll}
-5 & 9 & 15 & -3
\end{array}\right)\left(\begin{array}{l}
\mathcal{O}_{L^2 L^{\dagger+} D^2, 1}^{(p)} \\
\mathcal{O}_{L^2 L^{\dagger 2} D^2, 2}^{(p)} \\
\mathcal{O}_{L^2 L^{\dagger 2} D^2, 3}^{(p)} \\
\mathcal{O}_{L^2 L^{\dagger} D^2, 4}^{(p)}
\end{array}\right) \\
&
\end{aligned}
$$
\textbf{UV states} $\left(Spin, S U(3)_c, S U(2)_w, U(1)_y\right)=(1,1,3,0): g_{p_1 p_3}\left(\tau^I\right)_{i_3}^{i_1} \mathcal{W}_0^{\mu I}\left(L_{p_1 i_1} \sigma_\mu L_{p_3}^{\dagger i_3}\right)$
$$
\mathcal{L}_{\mathrm{UV}}=\frac{1}{2} \mathcal{W}_{0 \mu}^I\left(\square+M^2\right) \mathcal{W}_0^{\mu I}+g_{p_1 p_3}\left(\tau^I\right)_{i_3}^{i_1} \mathcal{W}_0^{\mu I}\left(L_{p_1 i_1} \sigma_\mu L_{p_3}^{\dagger i_3}\right)
$$
EOM of $\mathcal{W}_{0 \mu}^I$
$$
\begin{aligned}
 \mathcal{W}_{0 \mu}^I&=-\frac{g_{p_1 p_3}\left(\tau^I\right)_{i_3}^{i_1}\left(L_{p_1 i_1} \sigma_\mu L_{p_3}^{\dagger i_3}\right)}{\left(\square+M^2\right)} \\
 \mathcal{L}_{\mathrm{EFT}}&=\frac{g_{p_1 p_3} g_{p_2 p_4}}{2 M^4}\left(\tau^I\right)_{i_3}^{i_1}\left(\tau^I\right)_{i_4}^{i_2}\left(L_{p_1 i_1} \sigma_\mu L_{p_3}^{\dagger i_3}\right) \square\left(L_{p_2 i_2} \sigma^\mu L_{p_4}^{\dagger i_4}\right) \\
& =\frac{g_{p_1 p_3} g_{p_2 p_4}}{M^4}\left(\tau^I\right)_{i_3}^{i_1}\left(\tau^I\right)_{i_4}^{i_2}\langle 12\rangle\langle 24\rangle[24][34] \\
& =-\frac{g_{p_1 p_3} g_{p_2 p_4}}{M^4}\left(2 \delta_{i_4}^{i_1} \delta_{i_3}^{i_2}-\delta_{i_3}^{i_1} \delta_{i_4}^{i_2}\right)\langle 13\rangle\langle 24\rangle[34]^2 \\
& =-\frac{g_{p_1 p_2} g_{p_3 p_4}^*}{M^2}\left(\begin{array}{llll}
0 & -1 & 0 & 2
\end{array}\right)\left(\begin{array}{l}
\mathcal{O}_{L^2 L^{\dagger+} D^2, 1}^{(y)} \\
\mathcal{O}_{L^2 L^{\dagger+2} D^2, 2}^{(y)} \\
\mathcal{O}_{L^2 L^{\dagger 2} D^2, 3} \\
\mathcal{O}_{L^2 L^{\dagger 2} D^2, 4}^{(y)}
\end{array}\right) \\
& =-\frac{g_{p_1 p_2} g_{p_3 p_4}^*}{M^2}\left(\begin{array}{llll}
1 & 3 & -3 & -1
\end{array}\right)\left(\begin{array}{l}
\mathcal{O}_{L^2 L^{\dagger} D^2, 1}^{(p)} \\
\mathcal{O}_{L^2 L^{\dagger} D^2, 2}^{(p)} \\
\mathcal{O}_{L^2 L^{\dagger 2} D^2, 3}^{(p)} \\
\mathcal{O}_{L^2 L^{\dagger} D^2, 4}^{(p)}
\end{array}\right) \\
&
\end{aligned}
$$
$ \textbf{UV states}\left(Spin, S U(3)_c, S U(2)_w, U(1)_y\right)=(2,1,1,0): g_{p_1 p_3} \delta_{i_3}^{i_1} \mathcal{G}^{\mu \nu}\left(L_{p_1 i_1} i \sigma_\mu \stackrel{\leftrightarrow}{D}_\nu L_{p_3}^{\dagger_3}\right) $
$$
\begin{aligned}
 \mathcal{L}_{\mathrm{EFT}}&=\frac{g_{p_1 p_3} g_{p_2 p_4}}{2 M^2} \delta_{i_3}^{i_1} \delta_{i_4}^{i_2}\left(g^{\mu \lambda} g^{\nu \rho}+g^{\nu \lambda} g^{\mu \rho}-\frac{2}{3} g^{\mu \nu} g^{\lambda \rho}\right)\left(L_{p_1 i_1} i \sigma_\mu \stackrel{\leftrightarrow}{D}_\nu L_{p_3}^{\dagger i_3}\right)\left(L_{p_2 i_2} i \sigma_\lambda \stackrel{\leftrightarrow}{D}_\rho L_{p_4}^{\dagger i_4}\right) \\
& =\frac{g_{p_1 p_3} g_{p_2 p_4}}{2 M^2} \delta_{i_3}^{i_1} \delta_{i_4}^{i_2}\left(-8\langle 12\rangle\langle 34\rangle[34]^2+6\langle 13\rangle\langle 24\rangle[34]^2\right) \\
& =\frac{g_{p_1 p_3} g_{p_2 p_4}}{M^2}\left(\begin{array}{llll}
-4 & 3 & 0 & 0
\end{array}\right)\left(\begin{array}{l}
\mathcal{O}_{L^2 L^{\dagger 2} D^2, 1}^{(y)} \\
\mathcal{O}_{L^2 L^{\dagger 2} D^2, 2}^{(y)} \\
\mathcal{O}_{L^2 L^{\dagger 2} D^2, 3} \\
\mathcal{O}_{L^2 L^{\dagger 2} D^2, 4}^{(y)}
\end{array}\right) \\
& =\frac{g_{p_1 p_3} g_{p_2 p_4}}{M^2}\left(\begin{array}{llll}
-5 & -3 & -5 & -3
\end{array}\right)\left(\begin{array}{l}
\mathcal{O}_{L^2 L^{\dagger 2} D^2, 1}^{(p)} \\
\mathcal{O}_{L^2 L^{\dagger 2} D^2, 2}^{(p)} \\
\mathcal{O}_{L^2 L^{\dagger 2} D^2, 3}^{(p)} \\
\mathcal{O}_{L^2 L^{\dagger} D^2, 4}^{(p)}
\end{array}\right) \\
&
\end{aligned}
$$
$\textbf{UV states}\left(Spin,SU(3)_c, S U(2)_w, U(1)_y\right)=(1,1,1,0): g_{p_1 p_3} \delta_{i_3}^{i_1} \mathcal{B}_0^\mu\left(L_{p_1 i_1} \sigma_\mu L_{p_3}^{i_3}\right) $
$$
\\
\begin{aligned}
 \mathcal{L}_{\mathrm{EFT}}&=\frac{g_{p_1 p_3} g_{p_2 p_4}}{2 M^4} \delta_{i_3}^{i_1} \delta_{i_4}^{i_2}\left(L_{p_1 i_1} \sigma_\mu L_{p_3}^{\dagger i_3}\right) \square\left(L_{p_2 i_2} \sigma^\mu L_{p_4}^{\dagger i_4}\right) \\
& =\frac{g_{p_1 p_3} g_{p_2 p_4}}{M^4} \delta_{i_3}^{i_1} \delta_{i_4}^{i_2}\langle 12\rangle\langle 24\rangle[24][34] \\
& =-\frac{g_{p_1 p_3} g_{p_2 p_4}}{M^4} \delta_{i_3}^{i_1} \delta_{i_4}^{i_2}\langle 13\rangle\langle 24\rangle[34]^2 \\
& =-\frac{g_{p_1 p_3} g_{p_2 p_4}}{M^2}\left(\begin{array}{llll}
0 & 1 & 0 & 0
\end{array}\right)\left(\begin{array}{l}
\mathcal{O}_{L^2 L^{\dagger 2} D^2, 1}^{(y)} \\
\mathcal{O}_{L^2 L^{\dagger 2} D^2, 2}^{(y)} \\
\mathcal{O}_{L^2 L^{\dagger} D^2, 3}^{(y)} \\
\mathcal{O}_{L^2 L^{\dagger 2} D^2, 4}^{(y)}
\end{array}\right) \\
& =-\frac{g_{p_1 p_3} g_{p_2 p_4}}{M^2}\left(\begin{array}{llll}
1 & -1 & 1 & -1
\end{array}\right)\left(\begin{array}{l}
\mathcal{O}_{L^2 L^{\dagger+2} D^2, 1}^{(p)} \\
\mathcal{O}_{L^2 L^{\dagger 2} D^2, 2}^{(p)} \\
\mathcal{O}_{L^2 L^{\dagger 2} D^2, 3}^{(p)} \\
\mathcal{O}_{L^2 L^{+2} D^2, 4}^{(p)}
\end{array}\right) \\
&
\end{aligned}
$$
